Cascade Model-based Propensity Estimation for Counterfactual Learning to Rank

Unbiased CLTR requires click propensities to compensate for the difference between user clicks and true relevance of search results via IPS. Current propensity estimation methods assume that user click behavior follows the PBM and estimate click propensities based on this assumption. However, in reality, user clicks often follow the CM, where users scan search results from top to bottom and where each next click depends on the previous one. In this cascade scenario, PBM-based estimates of propensities are not accurate, which, in turn, hurts CLTR performance. In this paper, we propose a propensity estimation method for the cascade scenario, called CM-IPS. We show that CM-IPS keeps CLTR performance close to the full-information performance in case the user clicks follow the CM, while PBM-based CLTR has a significant gap towards the full-information. The opposite is true if the user clicks follow PBM instead of the CM. Finally, we suggest a way to select between CM- and PBM-based propensity estimation methods based on historical user clicks.

==> sections/02-Notations.tex <==
% !TEX root =  ../main.tex 


\section{Notations}
\todo{I think it is best to put all the notation into a table and drop this section.}

For a \textit{query} $q$ and \textit{document} $D$, we show the vector representation of $\langle q,D \rangle$ pair by $x_{q,D}$ or simply $x$. For a $x$, $c_x\in\{0,1\}$ and $r_x\in\{0,1\}$ indicate the click and relevancy signals, respectively. Note that we only consider binary relevance as is common in the counterfactual/online learning to rank literature \todo{references?}.
Related to the clicks, $e_x\in\{0,1\}$ is used to represent wether or not $x$ was examined by the user.
$c_{x,j}$ and $e_{x,j}$ indicate the click and examination signal on position $j$. 
We use uppercase letters $C_{x,j}$ and $E_{x,j}$ to indicate the random variables of clicks and examinations.
We follow the famous examination hypothesis with the hard assumption that \textit{attractiveness} is equivalent to the \textit{relevance} to come up with $c_{x,j}=e_{x,j}\cdot r_{x}$, similar to \cite{joachims2017unbiased,ai2018unbiased}. $f(x)$ is the ranker function.
For a query $q$, $\mathcal{D}_q$ is defined to be the ordered set of all documents shown in the result page of $q$, and the corresponding set of $x_{q,D}$'s for $D\in\mathcal{D}_q$ is denoted by $\mathcal{X}_{q}$. Since this study considers a top-$k$ setting, it is always the case that $|\mathcal{D}_q|=|\mathcal{X}_{q}|=k$.

